Perturbation Theory and Techniques

Prepared for the Quantum Field Theory section of the Encyclopedia of Mathematical Physics, Elsevier, 2006. A brief introduction to the methodology and techniques of perturbative relativistic quantum field theory is presented.

==> pert1 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 4 0 1 0 7 50 0 15 0.000 1 0.0000 5775 5062 228 228 6000 5100 5550 5025
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 6375 4950 37 37 6413 4950 6338 4950
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 6225 5400 37 37 6263 5400 6188 5400
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 6000 4500 37 37 6038 4500 5963 4500
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 5250 4800 37 37 5288 4800 5213 4800
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 5250 4800 5550 4950
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 6000 4500 5850 4875
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 6375 4950 6000 5025
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 6225 5400 5925 5175
4 0 0 50 0 0 12 0.0000 2 15 45 5250 5100 .\001
4 0 0 50 0 0 12 0.0000 2 15 45 5325 5325 .\001
4 0 0 50 0 0 12 0.0000 2 15 45 5625 5550 .\001
4 0 0 50 0 0 12 0.0000 2 15 45 6000 5550 .\001
4 0 0 50 0 0 12 0.0000 2 195 1395 6075 4500 $\\scriptstyle{k_1}$\001
4 0 0 50 0 0 12 0.0000 2 195 1395 6300 5475 $\\scriptstyle{k_3}$\001
4 0 0 50 0 0 12 0.0000 2 195 1395 6450 5025 $\\scriptstyle{k_2}$\001
4 0 0 50 0 0 12 0.0000 2 195 1395 5025 4800 $\\scriptstyle{k_n}$\001
4 0 0 50 0 0 11 0.0000 2 180 2565 3225 5100 $\\tilde G^{(n)}(k_1,\\dots,k_n)~=~$\001


==> pert2 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 525 4275 37 37 563 4275 488 4275
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 75 3375 1125 3375
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 165 3957 540 4257
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 525 4275 375 4725
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 518 4286 893 4511
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 547 4302 922 4002
4 0 0 50 0 0 12 0.0000 2 195 1215 900 3300 $\\scriptstyle{p}$\001
4 0 0 50 0 0 11 0.0000 2 195 1395 0 3975 $\\scriptstyle{p_n}$\001
4 0 0 50 0 0 11 0.0000 2 15 45 300 4500 .\001
4 0 0 50 0 0 11 0.0000 2 195 1395 300 4800 $\\scriptstyle{p_3}$\001
4 0 0 50 0 0 11 0.0000 2 195 1395 975 4575 $\\scriptstyle{p_2}$\001
4 0 0 50 0 0 11 0.0000 2 15 45 150 4350 .\001
4 0 0 50 0 0 11 0.0000 2 15 45 150 4125 .\001
4 0 0 50 0 0 11 0.0000 2 195 6405 1275 3375 $\\displaystyle=~\\int\\frac{\\dd^{d+1}p}{(2\\pi)^{d+1}}~\\frac\\ii{p^2-m^2+\\ii\\epsilon} \\ , $\001
4 0 0 50 0 0 11 0.0000 2 195 4080 1275 4275 $=~\\ii g~(2\\pi)^{d+1}~\\delta^{(d+1)}(p_1+\\dots+ p_n)$\001
4 0 0 50 0 0 11 0.0000 2 195 1395 975 3975 $\\scriptstyle{p_1}$\001


==> pert3 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3356 3553 237 237 3356 3553 3131 3478
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 3600 3600 4500 3600
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 2250 3600 3150 3600
4 0 0 50 0 0 12 0.0000 2 195 1080 2250 3525 $\\scriptstyle k$\001
4 0 0 50 0 0 12 0.0000 2 195 1080 4350 3525 $\\scriptstyle k$\001
4 0 0 50 0 0 11 0.0000 2 135 255 3225 3600 1PI\001
4 0 0 50 0 0 11 0.0000 2 195 1125 4650 3600 $=:~\\Sigma(k)$\001


==> pert4 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 2615 4204 237 237 2615 4204 2390 4129
1 3 0 1 0 7 50 0 15 0.000 1 0.0000 2148 2843 237 237 2148 2843 1923 2768
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3975 4200 237 237 3975 4200 3750 4125
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 3975 3600 237 237 3975 3600 3750 3525
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 1050 3600 1950 3600
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 1500 4200 2400 4200
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 2850 4200 3750 4200
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 4200 4200 5100 4200
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 4200 3600 5100 3600
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 2850 3600 3750 3600
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 2400 2850 3300 2850
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 0 0 2
	 975 2850 1875 2850
4 0 0 50 0 0 12 0.0000 2 195 1080 1350 3525 $\\scriptstyle k$\001
4 0 0 50 0 0 12 0.0000 2 195 1080 1575 4125 $\\scriptstyle k$\001
4 0 0 50 0 0 12 0.0000 2 195 1080 3300 4125 $\\scriptstyle k$\001
4 0 0 50 0 0 12 0.0000 2 195 1080 4875 4125 $\\scriptstyle k$\001
4 0 0 50 0 0 12 0.0000 2 195 1080 4950 3525 $\\scriptstyle k$\001
4 0 0 50 0 0 12 0.0000 2 195 1080 2925 3525 $\\scriptstyle k$\001
4 0 0 50 0 0 12 0.0000 2 195 1080 3150 2775 $\\scriptstyle k$\001
4 0 0 50 0 0 12 0.0000 2 195 1080 1050 2775 $\\scriptstyle k$\001
4 0 0 50 0 0 11 0.0000 2 165 285 675 3600 $=$\001
4 0 0 50 0 0 11 0.0000 2 135 255 2475 4275 1PI\001
4 0 0 50 0 0 11 0.0000 2 135 255 3825 4275 1PI\001
4 0 0 50 0 0 11 0.0000 2 165 285 2325 3600 $+$\001
4 0 0 50 0 0 11 0.0000 2 165 285 1050 4200 $+$\001
4 0 0 50 0 0 11 0.0000 2 165 720 5325 4200 $+~\\dots$\001
4 0 0 50 0 0 11 0.0000 2 195 3390 675 4875 $\\displaystyle=~\\frac\\ii{k^2-m^2-\\Sigma(k)}$\001
4 0 0 50 0 0 11 0.0000 2 135 255 3825 3675 1PI\001
4 0 0 50 0 0 11 0.0000 2 180 765 150 2850 $G(k)~:=$\001


==> pert5 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 3675 4425 52 52 3713 4463 3638 4388
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 3075 4500 52 52 3113 4538 3038 4463
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 3225 5100 52 52 3263 5138 3188 5063
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 3787 4912 52 52 3825 4950 3750 4875
1 4 0 1 0 7 50 0 -1 0.000 1 0.0000 3412 4725 405 405 3750 4950 3075 4500
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 1 0 2
	2 1 1.00 60.00 120.00
	 3000 4725 3000 4650
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 1 0 2
	2 1 1.00 60.00 120.00
	 3525 5100 3450 5100
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 1 0 2
	2 1 1.00 60.00 120.00
	 3375 4350 3450 4350
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 1 0 2
	2 1 1.00 60.00 120.00
	 3825 4800 3825 4875
4 0 0 50 0 0 11 0.0000 2 15 45 2850 4725 .\001
4 0 0 50 0 0 11 0.0000 2 15 45 2925 4950 .\001
4 0 0 50 0 0 11 0.0000 2 15 45 3075 5100 .\001
4 0 0 50 0 0 11 0.0000 2 195 1515 3750 4425 $\\scriptstyle V(x_1)$\001
4 0 0 50 0 0 11 0.0000 2 195 1515 3150 5325 $\\scriptstyle V(x_3)$\001
4 0 0 50 0 0 11 0.0000 2 195 10230 4425 4800 $\\displaystyle=~(-)\\,\\prod_{i=1}^n\\,\\int\\dd^4x_i~\\tr\\prod_{j=1}^{n-1}\\Delta_F(x_j-x_{j+1})\\,V(x_{j+1})\\,\\Delta_F(x_{j+1}-x_{j+2}) \\ . $\001
4 0 0 50 0 0 11 0.0000 2 195 1515 2625 4575 $\\scriptstyle V(x_n)$\001
4 0 0 50 0 0 11 0.0000 2 195 1515 3900 5025 $\\scriptstyle V(x_2)$\001


==> pert6 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 4800 3450 37 37 4838 3450 4763 3450
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 1 0 2
	2 1 1.00 60.00 120.00
	 4575 3450 4350 3450
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4350 3450 5250 3450
2 1 0 1 0 7 50 0 0 0.000 0 0 -1 1 0 2
	2 1 1.00 60.00 120.00
	 5100 3450 4875 3450
3 0 0 1 0 7 50 0 -1 0.000 0 0 0 7
	 4725 3000 4875 3075 4725 3150 4875 3225 4725 3300 4875 3375
	 4800 3450
	 0.000 1.000 1.000 1.000 1.000 1.000 0.000
4 0 0 50 0 0 11 0.0000 2 195 1965 5400 3300 $=~-\\ii e\\,\\gamma_\\mu \\ . $\001
4 0 0 50 0 0 11 0.0000 2 195 1215 4800 3600 $\\scriptstyle\\mu$\001


==> pert7 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 1050 2250 37 37 1088 2250 1013 2250
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 1050 6150 37 37 1088 6150 1013 6150
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 1050 3900 37 37 1088 3900 1013 3900
2 1 1 1 0 7 50 0 0 4.000 0 0 -1 0 1 2
	2 1 1.00 60.00 120.00
	 1350 6150 1425 6150
2 1 0 1 0 7 50 0 0 4.000 0 0 -1 1 0 2
	2 1 1.00 60.00 120.00
	 675 2550 750 2475
2 1 0 1 0 7 50 0 0 4.000 0 0 -1 1 0 2
	2 1 1.00 60.00 120.00
	 975 1875 900 1950
2 1 0 1 0 7 50 0 0 4.000 0 0 -1 1 0 2
	2 1 1.00 60.00 120.00
	 975 5775 900 5850
2 1 0 1 0 7 50 0 0 4.000 0 0 -1 1 0 2
	2 1 1.00 60.00 120.00
	 1425 2550 1350 2475
2 1 1 1 0 7 50 0 0 4.000 0 0 -1 0 0 2
	 450 4950 1650 4950
2 1 1 1 0 7 50 0 0 4.000 0 0 -1 0 0 2
	 450 6150 1650 6150
2 1 1 1 0 7 50 0 0 4.000 0 0 -1 0 1 2
	2 1 1.00 60.00 120.00
	 525 6150 600 6150
3 0 0 1 0 7 50 0 -1 0.000 0 0 0 9
	 450 900 600 750 750 900 900 750 1050 900 1200 750
	 1350 900 1500 750 1650 900
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 0 0 9
	 1050 2250 900 2250 900 2400 750 2400 750 2550 600 2550
	 600 2700 450 2700 450 2850
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 0 0 9
	 1050 2250 1200 2250 1200 2400 1350 2400 1350 2550 1500 2550
	 1500 2700 1650 2700 1650 2850
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 0 0 6
	 1050 1500 900 1650 1050 1800 900 1950 1050 2100 1050 2250
	 0.000 1.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 0 0 9
	 1050 3900 1200 3900 1200 4050 1350 4050 1350 4200 1500 4200
	 1500 4350 1650 4350 1650 4500
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 0 0 9
	 1650 3300 1500 3300 1500 3450 1350 3450 1350 3600 1200 3600
	 1200 3750 1050 3750 1050 3900
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 0 0 9
	 1050 3900 900 3900 900 4050 750 4050 750 4200 600 4200
	 600 4350 450 4350 450 4500
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 0 0 6
	 1050 5400 900 5550 1050 5700 900 5850 1050 6000 1050 6150
	 0.000 1.000 1.000 1.000 1.000 0.000
3 0 0 1 0 7 50 0 -1 0.000 0 0 0 9
	 450 3300 600 3300 600 3450 750 3450 750 3600 900 3600
	 900 3750 1050 3750 1050 3900
	 0.000 1.000 1.000 1.000 1.000 1.000 1.000 1.000
	 0.000
4 0 0 50 0 0 11 0.0000 2 195 1350 225 825 $\\scriptstyle b,\\nu$\001
4 0 0 50 0 0 11 0.0000 2 195 1350 1575 4650 $\\scriptstyle b,\\nu$\001
4 0 0 50 0 0 11 0.0000 2 195 1665 300 4650 $\\scriptstyle c,\\lambda$\001
4 0 0 50 0 0 11 0.0000 2 195 1080 975 975 $\\scriptstyle k$\001
4 0 0 50 0 0 11 0.0000 2 195 1080 975 5100 $\\scriptstyle k$\001
4 0 0 50 0 0 11 0.0000 2 180 6720 2850 4050 $+f^{eac}\\,f^{ebd}\\,(\\eta_{\\mu\\nu}\\,\\eta_{\\lambda\\rho}-\\eta_{\\mu\\rho}\\,\\eta_{\\nu\\lambda})$\001
4 0 0 50 0 0 11 0.0000 2 195 7575 2850 3750 ${-\\ii e^2\\big[f^{eab}\\,f^{ecd}(\\eta_{\\mu\\lambda}\\,\\eta_{\\nu\\rho}-\\eta_{\\mu\\rho}\\,\\eta_{\\nu\\lambda})}$\001
4 0 0 50 0 0 11 0.0000 2 195 7140 5175 4050 ${+f^{ead}\\,f^{ebc}(\\eta_{\\mu\\nu}\\,\\eta_{\\lambda\\rho}-\\eta_{\\nu\\rho}\\,\\eta_{\\mu\\lambda})\\big]}$\001
4 0 0 50 0 0 11 0.0000 2 195 9645 2850 2325 ${e\\,f^{abc}\\,\\bigl[\\eta_{\\lambda\\mu}(p_\\nu-k_\\nu)+\\eta_{\\mu\\nu}(q_\\lambda-p_\\lambda)+\\eta_{\\nu\\lambda}(k_\\mu-q_\\mu)\\bigr]}$\001
4 0 0 50 0 0 11 0.0000 2 180 1635 2850 5850 ${e\\,k_\\mu\\,f^{abc}}$\001
4 0 0 50 0 0 11 0.0000 2 195 1380 1650 825 $\\scriptstyle a,\\mu$\001
4 0 0 50 0 0 11 0.0000 2 195 1800 900 1425 $\\scriptstyle c,\\lambda,k$\001
4 0 0 50 0 0 11 0.0000 2 195 1515 1575 2925 $\\scriptstyle a,\\mu,p$\001
4 0 0 50 0 0 11 0.0000 2 195 1485 300 2925 $\\scriptstyle b,\\nu,q$\001
4 0 0 50 0 0 11 0.0000 2 195 1410 225 3300 $\\scriptstyle d,\\rho$\001
4 0 0 50 0 0 11 0.0000 2 195 1380 1650 3300 $\\scriptstyle a,\\mu$\001
4 0 0 50 0 0 11 0.0000 2 195 1080 300 4950 $\\scriptstyle b$\001
4 0 0 50 0 0 11 0.0000 2 195 1515 900 5325 $\\scriptstyle a,\\mu,p$\001
4 0 0 50 0 0 11 0.0000 2 195 1215 1575 6300 $\\scriptstyle b,q$\001
4 0 0 50 0 0 11 0.0000 2 195 3930 2850 5025 $\\displaystyle{\\frac{\\ii\\delta^{ab}}{k^2+\\ii\\epsilon}}$\001
4 0 0 50 0 0 11 0.0000 2 195 1200 300 6300 $\\scriptstyle c,k$\001
4 0 0 50 0 0 11 0.0000 2 195 7950 2850 900 $\\displaystyle{-\\ii\\delta^{ab}\\,\\frac{\\eta_{\\mu\\nu}+(\\alpha-1)\\,\\frac{k_\\mu\\,k_\\nu}{k^2}}{k^2+\\ii\\epsilon}}$\001
4 0 0 50 0 0 11 0.0000 2 195 1065 1725 4950 $\\scriptstyle a$\001


==> pert8 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
5 1 0 1 0 7 50 0 -1 0.000 0 1 0 0 7055.357 3300.000 7125 2850 6600 3300 7125 3750
1 4 0 1 0 7 50 0 -1 0.000 1 0.0000 750 3337 452 452 1200 3300 300 3375
1 3 0 3 0 7 50 0 -1 0.000 1 0.0000 750 3300 168 168 750 3300 900 3225
1 4 0 3 0 7 50 0 0 0.000 1 0.0000 2250 3300 75 75 2325 3300 2175 3300
1 4 0 1 0 7 50 0 -1 0.000 1 0.0000 3525 3337 452 452 3975 3300 3075 3375
1 3 0 3 0 7 50 0 -1 0.000 1 0.0000 3525 3300 168 168 3525 3300 3675 3225
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 300 3300 37 37 338 3300 263 3300
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 750 3750 37 37 788 3750 713 3750
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 1200 3300 37 37 1238 3300 1163 3300
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 3525 3750 37 37 3563 3750 3488 3750
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 3525 2850 37 37 3563 2850 3488 2850
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 3975 3300 37 37 4013 3300 3938 3300
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 3075 3300 37 37 3113 3300 3038 3300
1 4 0 1 0 7 50 0 -1 0.000 1 0.0000 5399 3298 452 452 5849 3261 4949 3336
1 4 0 3 0 7 50 0 0 0.000 1 0.0000 4950 3300 75 75 5025 3300 4875 3300
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 5400 3750 37 37 5438 3750 5363 3750
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 5887 3300 37 37 5925 3300 5850 3300
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 5400 2850 37 37 5438 2850 5363 2850
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 6600 3300 37 37 6638 3300 6563 3300
1 3 0 3 0 7 50 0 -1 0.000 1 0.0000 7125 3300 168 168 7125 3300 7275 3225
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 7125 3750 37 37 7163 3750 7088 3750
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 7125 2850 37 37 7163 2850 7088 2850
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 2400 4350 37 37 2438 4350 2363 4350
1 4 0 3 0 7 50 0 0 0.000 1 0.0000 2850 4350 75 75 2925 4350 2775 4350
1 3 0 3 0 7 50 0 -1 0.000 1 0.0000 4190 4332 168 168 4190 4332 4340 4257
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 4012 4350 37 37 4050 4350 3975 4350
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 4350 4350 37 37 4388 4350 4313 4350
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 3300 4350 37 37 3338 4350 3263 4350
1 4 0 1 0 7 50 0 -1 0.000 1 0.0000 2845 4336 452 452 3295 4299 2395 4374
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 2850 3900 37 37 2888 3900 2813 3900
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 2850 4800 37 37 2888 4800 2813 4800
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 3525 3450 37 37 3563 3450 3488 3450
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 3525 3150 37 37 3563 3150 3488 3150
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 750 3150 37 37 788 3150 713 3150
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 750 3450 37 37 788 3450 713 3450
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 750 2850 37 37 788 2850 713 2850
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 7125 3150 37 37 7163 3150 7088 3150
1 4 0 1 0 7 50 0 0 0.000 1 0.0000 7125 3450 37 37 7163 3450 7088 3450
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 750 3525 750 3750
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 750 2850 750 3075
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 150 3300 300 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1200 3300 1350 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 1950 3300 2550 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3525 2850 3525 3075
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3525 3525 3525 3750
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 4800 3300 4950 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5850 3300 6000 3300
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7125 2850 7125 3075
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7125 3525 7125 3750
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2250 4350 2400 4350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3300 4350 3450 4350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2850 3900 2850 4800
4 0 0 50 0 0 11 0.0000 2 165 285 1575 3300 $=$\001
4 0 0 50 0 0 11 0.0000 2 165 285 4200 3300 $+$\001
4 0 0 50 0 0 11 0.0000 2 165 270 4500 3300 $2$\001
4 0 0 50 0 0 11 0.0000 2 165 285 1950 4350 $+$\001
4 0 0 50 0 0 11 0.0000 2 165 480 2775 3300 $\\star$\001
4 0 0 50 0 0 11 0.0000 2 165 480 6225 3300 $\\star$\001
4 0 0 50 0 0 11 0.0000 2 165 480 3675 4350 $\\star$\001


==> pert9 <==
#FIG 3.2
Landscape
Center
Inches
Letter  
100.00
Single
-2
1200 2
1 3 0 1 0 7 50 0 -1 0.000 1 0.0000 6750 3900 168 168 6750 3900 6600 3825
1 1 0 1 0 7 50 0 14 0.000 1 0.0000 1950 3900 525 375 1950 3900 1425 3525
1 1 0 1 0 7 50 0 20 0.000 1 0.0000 1950 3900 225 150 1950 3900 1725 3750
1 4 0 1 0 -1 50 0 20 0.000 1 0.0000 3450 3750 37 37 3488 3750 3413 3750
1 4 0 1 0 -1 50 0 20 0.000 1 0.0000 3750 3750 37 37 3788 3750 3713 3750
1 4 0 1 0 -1 50 0 20 0.000 1 0.0000 3750 4050 37 37 3788 4050 3713 4050
1 4 0 1 0 -1 50 0 20 0.000 1 0.0000 3450 4050 37 37 3488 4050 3413 4050
1 4 0 1 0 -1 50 0 20 0.000 1 0.0000 4950 3900 37 37 4988 3900 4913 3900
1 4 0 1 0 -1 50 0 20 0.000 1 0.0000 5250 3900 37 37 5288 3900 5213 3900
1 4 0 1 0 -1 50 0 20 0.000 1 0.0000 5400 3675 37 37 5438 3675 5363 3675
1 4 0 1 0 -1 50 0 20 0.000 1 0.0000 5400 4125 37 37 5438 4125 5363 4125
1 4 0 1 0 -1 50 0 20 0.000 1 0.0000 6450 3900 37 37 6488 3900 6413 3900
1 4 0 1 0 -1 50 0 20 0.000 1 0.0000 6600 3900 37 37 6638 3900 6563 3900
1 4 0 1 0 -1 50 0 20 0.000 1 0.0000 6900 3900 37 37 6938 3900 6863 3900
1 4 0 1 0 -1 50 0 20 0.000 1 0.0000 7050 3900 37 37 7088 3900 7013 3900
2 1 0 1 0 7 50 0 20 0.000 0 0 -1 0 0 2
	 2550 4350 2250 4050
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3150 3450 3450 3750
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3450 4050 3150 4350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3750 4050 4050 4350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 3750 3750 4050 3450
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 3
	 4650 3450 4950 3900 4650 4350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 3
	 4950 3900 5250 3900 5550 3450
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5250 3900 5550 4350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 5400 3675 5400 4125
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 3
	 6150 3450 6450 3900 6150 4350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 6450 3900 6600 3900
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 3
	 6900 3900 7050 3900 7350 3450
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 7050 3900 7350 4350
2 1 0 1 0 7 50 0 -1 0.000 0 0 -1 0 0 2
	 2250 3825 2550 3450
2 1 0 1 0 7 50 0 20 0.000 0 0 -1 0 0 2
	 1425 3525 1725 3825
2 1 0 1 0 7 50 0 20 0.000 0 0 -1 0 0 2
	 1350 3450 1425 3525
2 1 0 1 0 7 50 0 20 0.000 0 0 -1 0 0 2
	 1350 3450 1575 3675
2 1 0 1 0 7 50 0 20 0.000 0 0 -1 0 0 2
	 1425 4350 1725 4050
2 1 0 1 0 -1 50 0 -1 0.000 0 0 -1 0 0 5
	 3450 3750 3450 4050 3750 4050 3750 3750 3450 3750
4 0 0 50 0 0 11 0.0000 2 135 840 1650 3825 $\\mbf\\times$\001
4 0 0 50 0 0 11 0.0000 2 135 840 2175 3825 $\\mbf\\times$\001
4 0 0 50 0 0 11 0.0000 2 135 840 2175 4050 $\\mbf\\times$\001
4 0 0 50 0 0 11 0.0000 2 135 840 1650 4050 $\\mbf\\times$\001
4 0 0 50 0 0 11 0.0000 2 135 240 2775 3900 $=$\001
4 0 0 50 0 0 11 0.0000 2 135 240 4275 3900 $+$\001
4 0 0 50 0 0 11 0.0000 2 135 240 5775 3900 $+$\001
4 0 0 50 0 0 11 0.0000 2 135 735 7500 3900 $+\\dots \\ . $\001

